Truthful Multi-Parameter Auctions with Online Supply: an Impossible Combination

We study a basic auction design problem with online supply. There are two unit-demand bidders and two types of items. The first item type will arrive first for sure, and the second item type may or may not arrive. The auctioneer has to decide the allocation of an item immediately after each item arrives, but is allowed to compute payments after knowing how many items arrived. For this problem we show that there is no deterministic truthful and individually rational mechanism that, even with unbounded computational resources, gets any finite approximation factor to the optimal social welfare.

==> preamble.tex <==

\topmargin=-0.35in \topskip=0pt \headsep=15pt \oddsidemargin=0pt
\textheight=9in \textwidth=6.3in \voffset=0in


\usepackage{amsmath,amsfonts,graphpap,amscd,mathrsfs,graphicx,lscape}
\usepackage{amssymb,amstext,xspace}
\usepackage{float}
%\usepackage[]{caption}
%\usepackage{subcaption}

%\usepackage[ruled]{algorithm2e}
%\renewcommand{\algorithmcfname}{ALGORITHM}
%\SetAlFnt{\small}
%\SetAlCapFnt{\small}
%\SetAlCapNameFnt{\small}
%\SetAlCapHSkip{0pt}
%\IncMargin{-\parindent}

\usepackage{color}              % Need the color package
\usepackage[title,header]{appendix}

%\usepackage{color-edits}
%\addauthor{cd}{green}
%\addauthor{vs}{red}
%\addauthor{nd}{blue}

\usepackage{amsthm}

\usepackage{url}
\usepackage[dvipsnames,usenames,table]{xcolor}
%\usepackage[colorlinks=true,urlcolor=blue,linkcolor=RoyalBlue,citecolor=OliveGreen]{hyperref}
\usepackage{prettyref, cleveref}
\usepackage[numbers]{natbib}

\usepackage{times}
